Computing the gauge-invariant bubble nucleation rate in finite temperature effective field theory

A gauge-invariant framework for computing bubble nucleation rates at finite temperature in the presence of radiative barriers was presented and advocated for model-building and phenomenological studies in an accompanying article arXiv:2112.05472. Here, we detail this computation using the Abelian Higgs Model as an illustrative example. Subsequently, we recast this approach in the dimensionally-reduced high-temperature effective field theory for nucleation. This allows for including several higher order thermal resummations and furthermore delineate clearly the approach's limits of validity. This approach provides for robust perturbative treatments of bubble nucleation during possible first-order cosmic phase transitions, with implications for electroweak baryogenesis and production of a stochastic gravitational wave background. Furthermore, it yields a sound comparison between results of perturbative and non-perturbative computations.

==> dr/diags.4pt.gl1,gl1,gl1,gl1.g4.E.tex <==
		\frac{1}{1}\,g^{4}\,Y_{\phi}^{4}\bigg)

